Programmable Spectral Filter Arrays using Phase Spatial Light Modulator

Spatially varying spectral modulation can be implemented using a liquid crystal spatial light modulator (SLM) since it provides an array of liquid crystal cells, each of which can be purposed to act as a programmable spectral filter array. However, such an optical setup suffers from strong optical aberrations due to the unintended phase modulation, precluding spectral modulation at high spatial resolutions. In this work, we propose a novel computational approach for the practical implementation of phase SLMs for implementing spatially varying spectral filters. We provide a careful and systematic analysis of the aberrations arising out of phase SLMs for the purposes of spatially varying spectral modulation. The analysis naturally leads us to a set of "good patterns" that minimize the optical aberrations. We then train a deep network that overcomes any residual aberrations, thereby achieving ideal spectral modulation at high spatial resolution. We show a number of unique operating points with our prototype including dynamic spectral filtering, material classification, and single- and multi-image hyperspectral imaging.

==> restorenet.tex <==
\subsection{Restoration of Assorted Measurements}
\label{sec:restorenet}
%
%Non-constant SLM patterns produce distortions in the captured image since the spectral response of a filter is affected by those of its neighboring filters as discussed in the previous subsection. 
%
%An ideal capture that is possible with our setup, thus, corresponds to constant SLM patterns wherein spectral filters in all pixels are the same. 
%
%Hence, a ``clean'' non-constant capture would have pixel intensities as if they were captured in a homogeneous setup. 
%
%We wish to use a restoration system that would correct such a distorted measured image to a clean image corresponding to the simulated measurement.
%
Our goal is to learn a mapping that takes the distorted measurements and produce clean ``simulated" measurements. 
%
Since interactions between neighboring spatial filters are non-linear, and often spatially varying, simple models may not capture the non-idealities. We instead rely on a learning-based approach to produce accurate measurements.

% Since the aforementioned distortions do not correspond to traditional models of blur and noise, 
%Complex interactions between neighboring filters make these distortions hard to model using conventional techniques.
%
%Hence, we follow a machine learning approach wherein we train a neural network to rectify these distortions using distorted and clean data pairs captured with our optical setup. 
%%
%To this end, in addition to the measured image of a chosen pattern, we capture images using constant patterns of all 256 filters which correspond to a Nyquist scan. 
%
%We create the simulated measurement image by simply sampling the correct filter locations in the Nyquist scan. 
%
We design a single neural network that takes the measured image as input, for any spatially-varying pattern on the SLM that is also provided as input, and outputs the ``simulated" measurement for that pattern produced from the full scan data.
%We start by generating simulated measurements from the full scan that we detailed in the previous section. These simulated images form the output for our training pipeline.
%
%The inputs are the measurements from the sensor array.
%
%These two sets of images will serve as our training data pairs.
%
% Thus, we have two images in our hands, a measured image and a simulated image for the same pattern. 
%
% We consider the latter to be the ground-truth version of the former as if there were no neighborhood filter interactions on SLM.
% 
%The goal of our neural network is thus to map the measured image to the corresponding simulated image. 
%
%Further, our aim is to have a single network which will correct distortions for any type of pattern. 
%Our aim is to train a single neural network that can be used for correcting distortion for any pattern.
%
%We note that, in the measured image, (i) the distortion depends on the specific combination of filters in a pattern, and (ii) spatial location of each filter on the image plane.
% , and (iii) the texture information is preserved in the guide RGB image. 
%
To account for the spatially varying artifacts, we include the coordinates $(x, y)$, the pattern index $p$ to the inputs, in addition to the measured intensity at each pixel. 
%
Based on the recent works of \cite{vaswani:2017:attention} and \cite{mildenhall:2020:nerf} in positional encoding, we transform each of $x, y$, and $p$ into 64-length encoded vectors instead of using their original scalar values. 
%
Given a $pos \in \{x, y, p\}$, we use 
%
$[\cos{(pos \cdot f^{2i/N})},$ 
$\sin{(pos \cdot f^{2i/N})}]$, 
for $i = 0, \ldots, N/2-1$ with $N = 64$ and $f = 10^{-4}$
%
as the 64-length positional encoding vector as suggested by \cite{vaswani:2017:attention}. 
%
%This results in 64 input channels each for two coordinates and one pattern index. 
%
Thus, the input to the network consists of a measurement intensity channel, 
% three guide RGB channels, 
and 64 channels each for $x, y$ and $p$, resulting in a total of 193 channels, as shown in Figure \ref{fig:restore_net_arch}. 
%
The output of the network is a single restored image channel corresponding to the simulated measurement.

\paragraph{Network Architecture.} We use an encoder-decoder architecture similar to that of U-net proposed by \cite{ronneberger:2015:unet} with four downsampling and four upsampling blocks as shown in Figure \ref{fig:restore_net_arch}. The specifics of this network and how it was trained is provided in the supplement.


%The number of channels when passing through the downsampling blocks are 192, 384, 768, and 768, and the upsampling blocks have them in reverse. 
%%
%Each downsampling block comprises of a convolution layer of kernel size $3 \times 3$ followed by a convolution layer of kernel size $4 \times 4$ with two strides for the downsampling operation. 
%%
%Each upsampling block comprises of a convolution-transpose layer of kernel size $4 \times 4$ with two strides for upsampling operation followed by a convolution layer of kernel size $3 \times 3$. 
%%
%The input is first passed on to an input convolutional layer of kernel size $3 \times 3$, and then on to the downsampling and upsampling blocks, and finally to an output convolutional layer of kernel size $3 \times 3$. 
%%
%All convolutional layers use a reflection padding of one, and all use Leaky ReLU activation with a negative slope of 0.2 except the output layer which uses none.


\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/restore_net/restore_net_arch_without_guide_v2.pdf}
    \caption{\textbf{Restoration network architecture.} Our pattern-oblivious encoder-decoder architecture rectifies the distortions in the measurement image using positional codes based on coordinates and pattern index.}
    \label{fig:restore_net_arch}
\end{figure}


\begin{figure}%[ht!]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/restore_net/restore_net_outputs_without_guide_v4_psnr.pdf}
    \caption{\textbf{Restoration of measured image.} We show $128 \times 128$ patches of a scene from our test data. 
    % The guide RGB image patches are shown in (a). 
    Each row in the left and right page columns corresponds to some of the different patterns that we employed during capture. The simulated measurement in (a) is the ``ground-truth'' image for each pattern. The measured image in (b) is very much distorted as can be seen by its absolute difference with the simulated measurement in (c). Our restoration network cleans up the distortions and produces the restored measurement image shown in (d) which has much lower distortions as can seen in (e). The efficacy of our restoration network can also be seen from much higher reconstruction PSNR values which are shown as insets.}
    \label{fig:restore_net_outputs}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.475\textwidth]{figures/real/PatternSweepFig_v2/Pattern_Measurement.pdf}
    \caption{\textbf{Improvements from restoration.} The restoration network provides measurements that have a higher fidelity to the ideal model, by correcting for blur and vignetting introduced by impreciseness in the optical implementation. We can see that, across all 92 SLM patterns, it provides an improvement of 7 dB or higher, as compared to the raw measurements. The numbers shown here are averages, over all the test scenes.}
    \label{fig:restore_patterns}
\end{figure}

\begin{figure}%[ht!]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/restore_net/restore_net_outputs_without_guide_v4_psnr_Plants3.pdf}
    \caption{\textbf{Restoration of measured image for unseen patterns.} Our trained network successfully cleans up the distortions in the measured image even for completely unseen patterns such as for the checkerboard-like patterns shown here.}
    \label{fig:restore_net_outputs_unseen}
\end{figure}

\paragraph{Restoration.} During inference, we input the measured image along with the positional encoding channels (all as $1024 \times 1024$ images) to the trained network to get the restored image as output which will be used for hyperspectral image reconstruction. We show the results of our restoration network for a test scene which is not used in training and validation in Figure \ref{fig:restore_net_outputs}. 

\paragraph{Performance of the restoration strategy.} Figure \ref{fig:restore_patterns} evaluates the performance of the restoration network on a test set of seven scenes. 
%
We quantify the error between the simulated and restored measurements, averaged across the seven scenes, for each of the 92 patterns, and compare them to that of the error associated with the measured images.
%
We use peak signal-to-noise ratio (PSNR), measured in dB, as our choice of metric which is defined as:
\begin{equation}
%  \textrm{SNR }  = 20 \log_{10} \left( \frac{\| {\bf x} \|_2 }{\| {\bf x} - \widehat{{\bf x}} \|_2 } \right),
 \textrm{PSNR }  = 20 \log_{10} \left( \frac{ \| \bfx \|_\infty}{ \textrm{RMSE}({\bf x}; \widehat{{\bf x}})  } \right),
 \end{equation}
where ${{\bf x}}$ and ${\widehat{{\bf x}}}$ are the simulated image and the restored/measurement image, respectively, with an intensity range [0--1].
%
We observe an improvement that is often greater than 
%10 dB, 
7 dB, 
indicating significant increase in measurement fidelity to the simulated data once we apply the restoration network.

\paragraph{Restoration of unseen patterns.} Since our restoration network is trained with the pattern code as well as an input, it is capable of restoring unseen patterns as well. We show the restoration outputs of patterns, previously unseen during training, in Figure \ref{fig:restore_net_outputs_unseen}.
%
Our network successfully restores these patterns, albeit with a slight loss in performance as compared to the patterns used at training.
%
This indicates that our trained network does not merely memorize a pseudo-random distribution of the patterns present in the training set, but can generalize for any pattern.  
